Planar stick indices of some knotted graphs

Two isomorphic graphs can have inequivalent spatial embeddings in 3-space. In this way, an isomorphism class of graphs contains many spatial graph types. A common way to measure the complexity of a spatial graph type is to count the minimum number of straight sticks needed for its construction in 3-space. In this paper, we give estimates of this quantity by enumerating stick diagrams in a plane. In particular, we compute the planar stick indices of knotted graphs with low crossing numbers. We also show that if a bouquet graph or a theta-curve has the property that its proper subgraphs are all trivial, then the planar stick index must be at least seven.

==> chapter03.tex <==
%!TeX  root = main_eng.tex
\chapter{Main Theorems and Results}
This chapter introduces our 4 main theorems and discusses how to implement them to obtain the final result. We prove our four main theorems in the next chapter. The last section of this chapter shows the planar diagrams of knots.
\section{Three Main Theorems}
\begin{thm} \label{thm:thm1}
\cite{Adams} Let \(\cro[K]\) be the crossing number of a knot \(K\) and \(\pl[K]\) the planar stick index of knot \(K\). Then
\[ \frac{3+\sqrt{9 + 8\,\cro[K]}}{2} \leq \pl[K]. \]
\end{thm}
\begin{thm} \label{thm:thm2}
There are only two planar diagrams for knot \(K\) of \(\pl[K] = 5\). Shown in the following figure.
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.6]{Theorem_2.png}
    \caption{The only two planar diagrams.}
    \label{fig:31}
\end{figure}
\end{thm}
\begin{thm} \label{thm:thm3}
The maximum crossings of planar diagram for knot \(K\) of \(\pl[K] = 6\) is 7.
\end{thm}
\begin{thm} \label{thm:thm4}
There are only two different types of planar diagram for knot \(K\) of \(\pl[K] = 6\). Show in the following figure.
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.6]{Corollary_1.png}
    \caption{The only two different types of planar diagram.}
    \label{fig:32}
\end{figure}
\end{thm}
\section{Identifying Planar Sticks of Knots}
A non-trivial knot has crossing number at least 3. We deduce from theorem \ref{thm:thm1} that the least number of sticks required to construct the smallest planar diagram is 5. By using only 5 sticks, we can construct the two planar diagram of knots as shown in figure \ref{fig:31}. In figure \ref{fig:31}, we can see that the left diagram represents \(3_1\) while the right diagram represents \(5_1\). Theorem \ref{thm:thm2} tells us that there are only two planar diagrams for \(\pl[K] = 5\) and each diagram represents only one knot. Thus, we can now conclude that \(\pl[3_1] = 5\) and \(\pl[5_1] = 5\). \par
We now focus on theorem \ref{thm:thm4}. We can see that there are two types of planar diagram with 6 segments with all of the crossings are still undeclared. By considering all of the possible crossings of the left diagram in figure \ref{fig:32}, we obtain that this diagram represents \(3_1, 4_1, 5_2, 6_1,\) and \(7_4\). But we already know that we can construct \(3_1\) by using only \(5\) sticks. Thus, we can conclude that the planar stick index of \(4_1, 5_2, 6_1,\) and \(7_4\) is \(6\). Repeating the same method to the right diagram in figure \ref{fig:32}, we obtain that this diagram represents \(3_1, 4_1, 5_1, 5_2,\) and \(6_2\). But the only new knot obtained from this diagram is \(6_2\). Thus, the planar stick index of \(6_2\) is 6.
\begin{cor}
The planar stick index of \(3_1\) and \(5_1\) is 5, and the planar stick index of \(4_1, 5_2, 6_1, 6_2,\) and \(7_4\) is 6. The planar stick index of knots other than these knots must be at least \(7\).
\end{cor}
The next smallest knot we still did not know its planar stick index yet is \(6_3\). The crossings number of \(6_3\) is 6, by applying theorem \ref{thm:thm1}; we obtained that the planar stick index of \(6_3\) is at least 6. But we formerly know that the planar stick index of knots other than \(3_1, 4_1, 5_1, 5_2, 6_1, 6_2,\) and \(7_4\) is at least 7. That means if we can construct planar diagram of knots other than \(3_1, 4_1, 5_1, 5_2, 6_1, 6_2,\) and \(7_4\) using exactly 7 sticks, then the planar stick index of that knot is 7. \par
The following figure shows the planar diagram for \(6_3\) using only 7 sticks. Thus, we can conclude that the planar stick index of \(6_3\) is 7, namely \(\pl[6_3] = 7\).
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.6]{6-3.png}
    \caption{The planar diagram for \(6_3\).}
    \label{fig:33}
\end{figure} \par
In this report, we found a lot of planar diagrams of knots other than \(3_1, 4_1, 5_1, 5_2,\) \(6_1, 6_2,\) and \(7_4\) using exactly 7 sticks. We illustrate those diagrams in the next section.
\section{Results}
The following table shows the planar diagrams of knots which is the final result of this report. The table contains 7 columns which are knot, crossing number, lower bound 1, lower bound 2, upper bound, planar stick index and diagram. Lower bound 1 is calculated from theorem \ref{thm:thm1}, lower bound 2 is obtained from \(\pl[K] \geq 2 \operatorname{b}[K]+1\) which is theorem 2.4 from~\cite{Adams}, upper bound shows the bound calculated by \(\pl[K] \leq \operatorname{s}[K]-1\) which is theorem 2.1 from~\cite{Adams}. \\
\\
\begin{minipage}{1.0\textwidth}
    \centering
    \vspace{5mm}
    %\captionof{table}{The planar diagrams of knots.}
    \label{tab:table1}
    \begin{tabular}{ccccccc}
        \toprule
        \multirow{2}{*}{Knot} & {Crossing} 
        					 & {Lower} 
					 & {Lower} 
					 & {Upper}
					 & {Planar} 
					 & \multirow{2}{*}{Diagram} \\
        {} & {Number} & {Bound 1} & {Bound 2} & {Bound} & {Stick Index} & {} \\
        \midrule
        \(3_1\) & 3 & 5 & 5 & 5 & 5 & \parbox[c]{7em}{\includegraphics[scale=0.25]{3-1.png}}	\\
        \(4_1\) & 4 & 5 & 5 & 6 & 6 & \parbox[c]{7em}{\includegraphics[scale=0.25]{4-1.png}}	\\
        \(5_1\) & 5 & 5 & 5 & 7 & 5 & \parbox[c]{7em}{\includegraphics[scale=0.25]{5-1.png}}	\\
        \(5_2\) & 5 & 5 & 5 & 7 & 6 & \parbox[c]{7em}{\includegraphics[scale=0.25]{5-2.png}}	\\
      \\	
      \bottomrule
    \end{tabular}
\end{minipage}
\newpage
\noindent
\begin{minipage}{1.0\textwidth}
    \centering
    \vspace{5mm}
    %\captionof{table}{The planar diagrams of knots.}
    \label{tab:table1}
    \begin{tabular}{ccccccc}
        \toprule
        \multirow{2}{*}{Knot} & {Crossing} 
        					 & {Lower} 
					 & {Lower} 
					 & {Upper}
					 & {Planar} 
					 & \multirow{2}{*}{Diagram} \\
        {} & {Number} & {Bound 1} & {Bound 2} & {Bound} & {Stick Index} & {} \\
        \midrule
        \(6_1\) & 6 & 6 & 5 & 7 & 6 & \parbox[c]{7em}{\includegraphics[scale=0.25]{6-1.png}}	\\
        \(6_2\) & 6 & 6 & 5 & 7 & 6 & \parbox[c]{7em}{\includegraphics[scale=0.25]{6-2.png}}	\\
        \(6_3\) & 6 & 6 & 5 & 7 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{6-3.png}}	\\
        \(7_1\) & 7 & 6 & 5 & 8 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{7-1.png}}	\\
        \(7_2\) & 7 & 6 & 5 & 8 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{7-2.png}}	\\
        \(7_3\) & 7 & 6 & 5 & 8 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{7-3.png}}	\\
        \(7_4\) & 7 & 6 & 5 & 8 & 6 & \parbox[c]{7em}{\includegraphics[scale=0.25]{7-4.png}}	\\
      \\	
      \bottomrule
    \end{tabular}
\end{minipage}
\newpage
\noindent
\begin{minipage}{1.0\textwidth}
    \centering
    \vspace{5mm}
    %\captionof{table}{The planar diagrams of knots.}
    \label{tab:table1}
    \begin{tabular}{ccccccc}
        \toprule
        \multirow{2}{*}{Knot} & {Crossing} 
        					 & {Lower} 
					 & {Lower} 
					 & {Upper}
					 & {Planar} 
					 & \multirow{2}{*}{Diagram} \\
        {} & {Number} & {Bound 1} & {Bound 2} & {Bound} & {Stick Index} & {} \\
        \midrule
        \(7_5\) & 7 & 6 & 5 & 8 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{7-5.png}}	\\
        \(7_6\) & 7 & 6 & 5 & 8 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{7-6.png}}	\\
        \(7_7\) & 7 & 6 & 5 & 8 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{7-7.png}}	\\
        \(8_2\) & 8 & 6 & 5 & 9 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{8-2.png}}	\\
        \(8_4\) & 8 & 6 & 5 & 9 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{8-4.png}}	\\
        \(8_6\) & 8 & 6 & 5 & 9 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{8-6.png}}	\\
        \(8_7\) & 8 & 6 & 5 & 9 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{8-7.png}}	\\
      \\	
      \bottomrule
    \end{tabular}
\end{minipage}
\newpage
\noindent
\begin{minipage}{1.0\textwidth}
    \centering
    \vspace{5mm}
    %\captionof{table}{The planar diagrams of knots.}
    \label{tab:table1}
    \begin{tabular}{ccccccc}
        \toprule
        \multirow{2}{*}{Knot} & {Crossing} 
        					 & {Lower} 
					 & {Lower} 
					 & {Upper}
					 & {Planar} 
					 & \multirow{2}{*}{Diagram} \\
        {} & {Number} & {Bound 1} & {Bound 2} & {Bound} & {Stick Index} & {} \\
        \midrule
        \(8_8\) 	& 8 & 6 & 5 & 9 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{8-8.png}}	\\
        \(8_{19}\) 	& 8 & 6 & 7 & 7 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{8-19.png}}	\\
        \(8_{20}\) 	& 8 & 6 & 7 & 7 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{8-20.png}}	\\
        \(9_1\) 	& 9 & 6 & 5 & 9 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{9-1.png}}	\\
        \(9_6\) 	& 9 & 6 & 5 & 10 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{9-6.png}}	\\
        \(9_7\) 	& 9 & 6 & 5 & 9 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{9-7.png}}	\\
        \(9_9\) 	& 9 & 6 & 5 & 9 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{9-9.png}}	\\
      \\	
      \bottomrule
    \end{tabular}
\end{minipage}
\newpage
\noindent
\begin{minipage}{1.0\textwidth}
    \centering
    \vspace{5mm}
    %\captionof{table}{The planar diagrams of knots.}
    \label{tab:table1}
    \begin{tabular}{ccccccc}
        \toprule
        \multirow{2}{*}{Knot} & {Crossing} 
        					 & {Lower} 
					 & {Lower} 
					 & {Upper}
					 & {Planar} 
					 & \multirow{2}{*}{Diagram} \\
        {} & {Number} & {Bound 1} & {Bound 2} & {Bound} & {Stick Index} & {} \\
        \midrule
        \(9_{11}\) 	& 9 & 6 & 5 & 10 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{9-11.png}}	\\
        \(9_{20}\) 	& 9 & 6 & 5 & 9 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{9-20.png}}	\\
        \(9_{26}\) 	& 9 & 6 & 5 & 9 & 7 & \parbox[c]{7em}{\includegraphics[scale=0.25]{9-26.png}}	\\
      \\	
      \bottomrule
    \end{tabular}
\end{minipage}

==> chapter04.tex <==
%!TeX  root = main_eng.tex
\chapter{Proof of Main Theorems}
\section{Proof of Theorem 3.1.1}
\begin{proof}
Start by considering the planar stick diagram of a knot \(K\) with \(\pl[K] = n\) sticks. Each stick can only cross \(n-3\) other sticks at a time, by excluding two from the two sticks adjacent to it and one from itself. The upper bound of the number of self-intersections (which is at least \(\cro[K]\)) is \(\frac{1}{2}(n)(n-3)\), obtained from basic combinatorics. Thus, by rearranging \(\cro[K] \leq \frac{1}{2}(n)(n-3)\) gives us the desired inequality.
\end{proof}
\section{Proof of Theorem 3.1.2}
\begin{proof}
We prove this theorem by construction. Start by having 5 sticks, we place the first stick horizontally as shown in the following figure.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{421.png}
    \caption{Placing the first stick.}
    \label{fig:421}
\end{figure}
\noindent 
The second stick must adjacent to the first stick. So, there are a lot of ways to place the second stick. Without loss of generality, we place the second stick obliquely up as shown in the following figure.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{422.png}
    \caption{Placing the second stick.}
    \label{fig:422}
\end{figure}
\noindent 
To avoid the trivial knot in the final result, we must place the third stick as if it is going to intersect the first stick. Here we have two ways to place, one intersect the first stick and the another one is not.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{423.png}
    \caption{Placing the third stick.}
    \label{fig:423}
\end{figure}
\noindent 
We again avoiding to construct trivial knot, so, the fourth stick must place as in the following figure.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{424.png}
    \caption{Placing the fourth stick.}
    \label{fig:424}
\end{figure}
\noindent 
The last stick connecting the fourth and the first stick.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{425.png}
    \caption{Placing the fifth stick.}
    \label{fig:425}
\end{figure}
\noindent 
Therefore, by construction there are only two planar diagrams. Planar diagram other than these two diagram would be a planar diagram for trivial knot.
\end{proof} \newpage
\section{Proof of Theorem 3.1.3}
\begin{proof}
We prove this theorem by construction and observation. Start by having 6 sticks. First, we place the first stick horizontally as shown in the following figure.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{431.png}
    \caption{Placing the first stick.}
    \label{fig:431}
\end{figure}
\noindent The second stick must adjacent to the first stick. We can see that there are a lot of ways to place the second stick. Without loss of generality, we place the second stick obliquely up as shown in the following figure.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{432.png}
    \caption{Placing the second stick.}
    \label{fig:432}
\end{figure}
\noindent To obtain the most crossing in the final diagram, the third stick must intersect the first stick.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.45]{433.png}
    \caption{Placing the third stick.}
    \label{fig:433}
\end{figure}
\noindent Because we want the final diagram have crossings as much as possible. So, the fourth stick must be placed intersecting the first and the second sticks.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.45]{434.png}
    \caption{Placing the fourth stick.}
    \label{fig:434}
\end{figure}
\noindent There are two different ways to place the fifth stick. Show in the following figure.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.45]{435.png}
    \caption{Placing the fifth stick.}
    \label{fig:435}
\end{figure}
\noindent We see that the first way is not a desired diagram, because the crossing where the fifth stick intersect the first stick can be untangled and gives us just a diagram of 5 sticks. So, we will use the second way instead.
The following is our final diagram after placing the last stick.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.4]{436.png}
    \caption{Placing the sixth stick.}
    \label{fig:436}
\end{figure}
Now, we focus on the two emphasized sticks. Which are the second stick and the sixth stick. Show in the following figure.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.4]{437.png}
    \caption{Two emphasizing sticks.}
    \label{fig:437}
\end{figure}
\noindent We know that the upper bound of the number of self-intersections is \(\frac{1}{2}(n)(n-3)\) where \(n\) is the number of sticks. By taking \(n = 6\), we have that the upper bound is 9. Back to our final diagram, we see that the crossings occur on the second and sixth sticks were only 2 crossings. But we also know that each stick can cross \(n - 3 = 6 - 3 = 3\) other stick at a time. So, we lose 1 crossing from these two sticks. Therefore, the maximum crossings of planar diagram for knot \(K\) of \(\pl[K] = 6\) is \(9 - 2 = 7\).
\end{proof}
\section{Proof of Theorem 3.1.4}
\begin{proof}
We prove this theorem by construction. By having 6 sticks, we place the first stick horizontally as shown below.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{441.png}
    \caption{Placing the first stick.}
    \label{fig:441}
\end{figure}
Without loss of generality, we place the second stick vertically.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{442.png}
    \caption{Placing the second stick.}
    \label{fig:442}
\end{figure}
We used 2 sticks out of 6 sticks, means that we have 4 sticks left. We know that the sixth stick must connect another endpoint of the first stick. So, the number of sticks that need to cross the first stick is 3. And we label the positions of the crossings occur as shown in the following figure.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{443.png}
    \caption{Labeling three positions of crossings.}
    \label{fig:443}
\end{figure}
These 3 dots indicate the order of stick passing through the first stick. For example, if we label the first dot by 3, the middle dot by 4, and the last dot by 5 (denoted by \((3\,4\,5)\)) we obtain the following diagram.
\begin{figure}[H]
    \centering
    \includegraphics[scale=0.5]{444.png}
    \caption{Diagram of \((3\,4\,5)\).}
    \label{fig:444}
\end{figure}
By using this method to construct diagrams, we will obtain 6 diagrams (from permuting those 3 dots) show in the following table. \\
\begin{minipage}{1.0\textwidth}
    \centering
    \vspace{5mm}
    %\captionof{table}{The planar diagrams of knots.}
    \label{tab:table2}
    \begin{tabular}{ccccccc}
        \toprule
        {No.} & {Notation} & {Diagram} &  & {No.} & {Notation} & {Diagram} \\
        \midrule
      \(1\)	& (\(3\,4\,5\)) &	\parbox[c]{7em}{\includegraphics[scale=0.25]{Form_1.png}} &&	
      \(2\)	& (\(4\,3\,5\)) &	\parbox[c]{7em}{\includegraphics[scale=0.25]{Form_2.png}}	\\
      \(3\)	& (\(3\,5\,4\)) &	\parbox[c]{7em}{\includegraphics[scale=0.25]{Form_3.png}} &&
      \(4\)	& (\(4\,5\,3\)) &	\parbox[c]{7em}{\includegraphics[scale=0.25]{Form_4.png}}	\\
      \(5\)	& (\(5\,3\,4\)) &	\parbox[c]{7em}{\includegraphics[scale=0.25]{Form_5.png}} &&
      \(6\)	& (\(5\,4\,3\)) &	\parbox[c]{7em}{\includegraphics[scale=0.25]{Form_6.png}}	\\
      \\	
      \bottomrule
    \end{tabular}
\end{minipage} \\ \\ \\
We can see that diagrams number 4 and 5 are just the planar diagram of knot \(K\) where \(\pl[K] = 5\) and the diagram number 6 is trivial. We have 3 diagrams left which are number 1, 2, and 3. We again see that if we rotate the diagram number 3 by \(180^{\circ}\), we would obtain the same diagram as number 2. Another reason to tell the diagram number 3 is the same diagram as the number 2 is if we rotate the diagram number 3 by \(180^{\circ}\) and re-denoting its notation, we will obtain the same notation as the diagram number 2 which is \((4\,3\,5)\). Therefore, we have only 2 different diagrams left which are number 1 and 2.
\end{proof}
